Lepton-Nucleus Scattering Measurements for Neutrino Interactions and Oscillations

Currently running and forthcoming precision neutrino oscillation experiments aim to unambiguously determine the neutrino mass ordering, the charge-parity violating phase in the lepton sector and the possible existence of physics Beyond the Standard Model. To have an understanding of all the effects necessary for the success of these experiments, lepton-nucleus interactions must be modeled in unprecedented detail. With this thesis, expertise in both neutrino and electron cross-section modeling and analysis was leveraged in order to make fundamental and critical improvements to our understanding of these interactions. The outlined work takes a significant step towards this high-precision measurement era with three complementary approaches. Cross sections are reported using neutrino data sets from the MicroBooNE liquid argon time projection chamber detector at Fermi National Laboratory, as well as electron scattering data from the CLAS detector at Thomas Jefferson National Laboratory. Furthermore, the modeling development of the commonly used GENIE event generator is presented.

==> READMEs/README_bibliography.tex <==
%% This file gives an overview on what you will need to do to create a
%% bibliographic database for references, as well as create the actual
%% bibliography for your thesis.

%% You should not need to touch the file biblio.tex.  This merely tells
%% latex to look for the file with the bibliographic info.  The file you
%% want to edit is main.bib.  For each entry, use the appropriate style
%% as designated in the file.

%% Citing your references:

%% When you cite a reference, you need to use the ``key'' you declare in
%% main.bib for the entry.  No one ever sees the keys, but you'll want to
%% use something you will easily remember.  For instance, if you had an
%% entry with:

%% 	   key=geer1

%% Then you would use \cite{geer1} to reference it within your thesis.

%% NOTE: You can not include references in your bibliography that are
%% never cited in your paper by default. If you need to do this, create a
%% key for the entry and at the end of your thesis include the line:

%% \nocite{key}

%% This should be done for every entry which is not explicitly cited.



==> READMEs/README_main.tex <==
%% This file explains the options available to you for editing the file
%% main.tex.

%% The commands in this file allow you to specify options such as
%% spacing, double-sided printing, a draft copy, etc.   By default, 12pt
%% and lgrind are included; lgrind is the 2e style for including code in
%% your thesis.

%% \documentclass[12pt]{mitthesis}
%% \usepackage{lgrind}
%% \pagestyle{plain}

%% You can add options in the documentclass line as follows:

%% 	o  singlespace
%% 	\documentclass[12pt,singlespace]{mitthesis}
	
%% 	o  twoside
%% 	\documentclass[12pt,twoside]{mitthesis}

%% 	o  draft   (make sure to change the pagestyle to drafthead as well)
%% 	\documentclass[12pt,draft]{mitthesis}
%% 	\usepackage{lgrind}
%% 	\pagestyle{drafthead}

%% 	o vi   (for course vi and course viii theses)
%% 	\documentclass[12pt,vi]{mitthesis}

%% Any options you would use for report.sty will work here as well.


%% You should not need to change the first three lines and last two lines
%% below.  Be sure to include an \include command for each file you are
%% including in your thesis.
  
%% \include{cover}
%% \pagestyle{plain}
%% \include{contents}
%% \include{chap1}
%% \include{chap2}
%% \appendix
%% \include{appa}
%% \include{appb}
%% \include{biblio}
%% \end{document}

%% Comment: to include appendices use a single \appendix command followed 
%% by a number of \include{} commands as many files as needed, each of 
%% which should contain a \chapter{} command for the appendix title.


==> READMEs/README_text.tex <==
%% This file includes the basic commands you will need to use within each
%% chapter of your thesis.

%% The file chap1.tex is a sample first chapter.  To get started, you may
%% just want to replace the text and commands in that file as needed.  In
%% general though, for each new chapter you want to do the following:

%% 	o Make sure the name has the extension .tex .  Otherwise, you
%% 	can call it anything you want.  For ease of use, all the
%% 	examples use chap1, chap2, etc.

%% 	o Add a line to the file main.tex that reads:
%% 	\include{yourfilename}

%% 	This should not include the .tex extension, because latex
%% 	assumes that is there.

%% Basic syntax:

%% 	o The first line of each chapter should be:
%% 	\chapter{Chapter Title}

%% 	o To start a new section (labeled chap#.sec# -- as in 1.1,
%% 	1.2, etc):
%% 	\section{Section Heading}

%% 	You can also include subsections:
%% 	\subsection{Heading}




==> conclusions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\chapter{Conclusions}\label{conclusions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> signature.tex <==
% -*- Mode:TeX -*-
%
% Some departments (e.g. Chemistry) require an additional cover page
% with signatures of the thesis committee.  Please check with your
% thesis advisor or other appropriate person to determine if such a 
% page is required for your thesis.  
%
% If you choose not to use the "titlepage" environment, a \newpage
% commands, and several \vspace{\fill} commands may be necessary to
% achieve the required spacing.  The \signature command is defined in
% the "mitthesis" class
%
% The following sample appears courtesy of Ben Kaduk <kaduk@mit.edu> and
% was used in his June 2012 doctoral thesis in Chemistry. 

\begin{titlepage}
\begin{large}
This doctoral thesis has been examined by a Committee of the Department
of Chemistry as follows:

\signature{Professor Jianshu Cao}{Chairman, Thesis Committee \\
   Professor of Chemistry}

\signature{Professor Troy Van Voorhis}{Thesis Supervisor \\
   Associate Professor of Chemistry}

\signature{Professor Robert W. Field}{Member, Thesis Committee \\
   Haslam and Dewey Professor of Chemistry}
\end{large}
\end{titlepage}


